Hybrid OpenMP/MPI programs for solving the time-dependent Gross-Pitaevskii equation in a fully anisotropic trap

We present hybrid OpenMP/MPI (Open Multi-Processing/Message Passing Interface) parallelized versions of earlier published C programs (D. Vudragovic et al., Comput. Phys. Commun. 183, 2021 (2012)) for calculating both stationary and non-stationary solutions of the time-dependent Gross-Pitaevskii (GP) equation in three spatial dimensions. The GP equation describes the properties of dilute Bose-Einstein condensates at ultra-cold temperatures. Hybrid versions of programs use the same algorithms as the C ones, involving real- and imaginary-time propagation based on a split-step Crank-Nicolson method, but consider only a fully-anisotropic three-dimensional GP equation, where algorithmic complexity for large grid sizes necessitates parallelization in order to reduce execution time and/or memory requirements per node. Since distributed memory approach is required to address the latter, we combine MPI programing paradigm with existing OpenMP codes, thus creating fully flexible parallelism within a combined distributed/shared memory model, suitable for different modern computer architectures. The two presented C/OpenMP/MPI programs for real- and imaginary-time propagation are optimized and accompanied by a customizable makefile. We present typical scalability results for the provided OpenMP/MPI codes and demonstrate almost linear speedup until inter-process communication time starts to dominate over calculation time per iteration. Such a scalability study is necessary for large grid sizes in order to determine optimal number of MPI nodes and OpenMP threads per node.

==> GP-SCL-HYB/makefile <==
# GP-SCL-HYB codes are developed by:
# 
# Bogdan Sataric
# (Faculty of Technical Sciences, University of Novi Sad, Serbia)
#
# Vladimir Slavnic, Aleksandar Belic, Antun Balaz
# (Institute of Physics Belgrade, Serbia, http://www.scl.rs/)
# 
# Paulsamy Muruganandam
# (Bharathidasan University, Tamil Nadu, India)
# 
# Sadhan K. Adhikari
# (UNESP - Sao Paulo State University, Brazil)
# 
# 
# Public use and modification of this code are allowed provided that the
# following papers are cited:
# [1] B. Sataric et al., Comput. Phys. Commun. 200 (2016) 411;
# [2] P. Muruganandam and S. K. Adhikari, Comput. Phys. Commun. 180 (2009) 1888;
# [3] D. Vudragovic et al., Comput. Phys. Commun. 183 (2012) 2021.
#
# The authors would be grateful for all information and/or comments regarding
# the use of the code.

CC = mpicc
CFLAGS = -O5
OMPFLAGS = -fopenmp
LIBS = -lm
OMPLIBS = -lpthread

IMAGTIME_TARGETS=imagtime3d-hyb
IMAGTIME_OBJECTS=$(IMAGTIME_TARGETS:=.o)

REALTIME_TARGETS=realtime3d-hyb
REALTIME_OBJECTS=$(REALTIME_TARGETS:=.o)

UTIL_TARGETS=diffint mem cfg misc
UTIL_OBJECTS=$(UTIL_TARGETS:=.o)

all: $(IMAGTIME_TARGETS) $(REALTIME_TARGETS)
	@rm -rf $(UTIL_OBJECTS)

imagtime3d: $(IMAGTIME_TARGETS)
	@rm -rf $(UTIL_OBJECTS)
	
realtime3d: $(REALTIME_TARGETS)
	@rm -rf $(UTIL_OBJECTS)
	
help: readme.txt
	less $^

$(IMAGTIME_TARGETS): % : $(UTIL_OBJECTS) %.o
	$(CC) $(CFLAGS) $(OMPFLAGS) -o $@ $@.o $(UTIL_OBJECTS) $(LIBS) $(OMPLIBS)
	@rm -rf $@.o
	
$(REALTIME_TARGETS): % : $(UTIL_OBJECTS) %.o
	$(CC) $(CFLAGS) $(OMPFLAGS) -o $@ $@.o $(UTIL_OBJECTS) $(LIBS) $(OMPLIBS)
	@rm -rf $@.o
	
$(IMAGTIME_OBJECTS): %.o:
	$(CC) $(CFLAGS) $(OMPFLAGS) -c src/$*/$*.c -o $@

$(REALTIME_OBJECTS): %.o:
	$(CC) $(CFLAGS) $(OMPFLAGS) -c src/$*/$*.c -o $@

$(UTIL_OBJECTS): %.o:
	$(CC) $(CFLAGS) -c src/util/$*.c -o $@
	
clean:
	@rm -rf $(IMAGTIME_TARGETS) $(REALTIME_TARGETS) \
           $(IMAGTIME_OBJECTS) $(REALTIME_OBJECTS) \
           $(UTIL_OBJECTS)

